Maximizing Fair Content Spread via Edge Suggestion in Social Networks

Content spread inequity is a potential unfairness issue in online social networks, disparately impacting minority groups. In this paper, we view friendship suggestion, a common feature in social network platforms, as an opportunity to achieve an equitable spread of content. In particular, we propose to suggest a subset of potential edges (currently not existing in the network but likely to be accepted) that maximizes content spread while achieving fairness. Instead of re-engineering the existing systems, our proposal builds a fairness wrapper on top of the existing friendship suggestion components. We prove the problem is NP-hard and inapproximable in polynomial time unless P = NP. Therefore, allowing relaxation of the fairness constraint, we propose an algorithm based on LP-relaxation and randomized rounding with fixed approximation ratios on fairness and content spread. We provide multiple optimizations, further improving the performance of our algorithm in practice. Besides, we propose a scalable algorithm that dynamically adds subsets of nodes, chosen via iterative sampling, and solves smaller problems corresponding to these nodes. Besides theoretical analysis, we conduct comprehensive experiments on real and synthetic data sets. Across different settings, our algorithms found solutions with nearzero unfairness while significantly increasing the content spread. Our scalable algorithm could process a graph with half a million nodes on a single machine, reducing the unfairness to around 0.0004 while lifting content spread by 43%.

==> FireF-eg-fig.tex <==
\begin{figure*}[!ht] 
    %\begin{minipage}
    \begin{subfigure}[t]{0.32\linewidth}
        	\centering
        	\includegraphics[width=\textwidth]{figs/scale1.pdf} 
        	\caption{Initial Stage}
            \label{fig:sc:1}
    %\end{minipage}
    \end{subfigure}
    \hfill
    %\begin{minipage}
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        	\includegraphics[width =\textwidth]{figs/figure2.pdf} 
        	\caption{Iteration 1}
            \label{fig:sc:2}
    %\end{minipage} 
    \end{subfigure}
    \hfill
    %\begin{minipage}
    \begin{subfigure}[t]{0.32\linewidth}
        	\centering
        	\includegraphics[width =\textwidth]{figs/figure3.pdf}
        	\caption{Iteration 2}
            \label{fig:sc:3}
    %\end{minipage}
    \end{subfigure}
    \caption{Illustration of two iterations of the Forest Fire algorithm on a toy graph with two content nodes (Fig~\ref{fig:sc:1}).}
    \label{fig:sc}
\end{figure*}  

==> archive/methods.tex <==
\section{The Randomized Approximation Algorithm}\label{sec:methods}
In previous section, we proved that \problem is NP-hard and provided some negative results about it.
Therefore, in this section, we turn our attention to designing an 
approximation algorithm for the \problem problem with provable guarantees both on the content spread and on fairness, if a valid solution exists.


In particular, our algorithm is LP-relaxation followed by randomized rounding.







In order to determine the RMPP content spread to each node without use of a maximum probability function, we instead consider what we call a "$\Delta$ probability" of each edge distance, based on the work by G\"uney~\cite{GUNEY2019589}. $\Delta$ probability is the increase in probability for decreasing the distance to a node, defined as the probability that a node receives content as distance $r$ minus the probability that a node receives content at distance $r+1$ (when $r$ is less than the largest distance from a source node on the graph or simply the actual probability if $r$ is the maximum distance). It should be noted that this requires the graph to be connected from the source nodes, and in practice the subset of nodes which are connected can be used if this is not the case.

To create an integer program with this concept, for each node $i$ and each possible distance $r$, we define an indicator $x_{ir}$, to indicate whether the node is reachable on a graph by an RMPP path of length $r$ or less. We compute this by assigning $x_{ir} \leq \sum_{j \in P_{ir}} y_j$, where $P_{ir}$ is all the edges $e_j$ for which $x_{ir}$ would be 1 for $G(V,E \cup \{e_j\})$ The linear equation $\Delta * X * W$ when maximized is then equal to the weighted RMPP content spread for a $G(V,E \cup E_p)$. The formal definition of the integer program is as follows.


\begin{figure}[!tb]
    % \centering
    \framebox[1.04\columnwidth]{
    \parbox{\columnwidth}{
    \begin{align*}
        \mbox{max}&\mbox{imize}~ \sum_{r=1}^{r_m} \delta_r \sum_{v_i\in V} {w_ix_{ir}}\\
        \mbox{sub}&\mbox{ject to} &~\\
        &\forall v_i\in V,r\in[1,r_m],~x_{ir} \leq \sum_{e_j \in P_{ir}} y_j\\
        &\forall  v_i\in V,~  \sum_{e_j \in edges(v_i)}y_j \leq k\\
        &\forall\gee_a, \gee_b\in \Gee,~ \frac{1}{|\gee_a|}\sum_{r=1}^{r_m} \delta_r\sum_{v_\ell \in \gee_a}{w_\ell x_{\ell r}} = \frac{1}{|\gee_b|}\sum_{r=1}^{r_m} \delta_r\sum_{v_\ell \in \gee_b}{w_\ell x_{\ell r}}\\
        &\forall  v_i\in V,~   0 \leq x_i \leq 1\\
        &\forall  e_j\in E_c,~  0 \leq y_j \leq 1 %y_j \in \{0,1\}
    \end{align*}}}
    \caption{LP-relaxation used for solving \problem problem.}
    \label{fig:LPRelax}
\end{figure}

\subsection{Linear Programming Approximation}

While an integer program can provide a best optimization value on integer inputs, a linear program provides a strictly equal or better optimization value with the relaxation that now the inputs can be any real number. This relaxation from the realm of integers to the realm of reals is known as an LP Relaxation\cite{schrijver1998theory}. A linear program is derived from the integer program by relaxing the inputs $\forall_j y_j \in \{0,1\}$ to be any real value between 0 and 1:

\begin{equation}\label{lp-constraint}
\forall_j 0 \leq y_j \leq 1
\end{equation}

By solving an Linear Programming problem, and performing a process called "randomized rounding" on the derived input values between zero and one to receive binary selections, it is possible to create an approximation algorithm of the original problem, often with theoretical guarantees\cite{raghavan1987randomized}. We introduce an approximation guaranteed LP relaxation to approximately solve Problem~\ref{def:equityspread}. We call this algorithm LP-Advanced, and later improve upon LP-Advanced to an algorithm LP-Optimized which removes unnecessary constraints from LP-Advanced without changing the expected output. 

LP-Advanced works in two stages. In the first stage, it pre-processes $P_{ir}$ sets by measuring the distance for each graph $\forall_{e_j \in E_c}\allowbreak G(V,E\cup\{e_j\})$, and including $e_j$ in any satisfying $P_{ir}$ set. Additionally the edges are collected into sets for each node $i$ if 1) the graph is directed and the edge is outgoing from $i$, or 2) if the graph is undirected and the edge is incident to the $i$. It then uses these values to solve the linear programming problem, yielding the optimal weights for edges $y^*$. Then randomized rounding is performed on these weights many times, yielding a collection of rounded $y^+$ edge sets. Among the $y^+$ sets, a small subset of the highest equity is selected, and from that subset a single set with the highest content spread is selected. In Section~\ref{sec:exp} we will demonstrate that this process gives us an answer that is not only theoretically guaranteed, but also near optimal.

The second stage addresses a shortfall of this model that occurs with what we call "downstream" edges. An edge is downstream of another edge if the shortest path to the source node of the downstream edge from a content node goes through the upstream edge. For any downstream edge, if the change in content spread is \emph{dominated} by the upstream edge, meaning the RMPP value of adding downstream edge has no impact on any node after the upstream edge, then the downstream edge is redundant, and there is often no incentive to include such edges.\ian{We need a figure here, this is hard to explain}. However, in the MIP and IC models, this edge may still have an impact. Accordingly we do two things. First, when calculating the best rounding, we use the MIP model. Second, the first stage will be repeated, adding the selected edges to the graph, and recalculating on the remaining viable edges. This continues until the feasible nodes (nodes for which $k$ edges have not been selected and still have non-selected incident candidate edges) falls beneath some threshold percentage of the initial feasible nodes, or no new edges are selected. At that point the second stage is complete, and the overall resultant set of selected edges is returned.

\begin{theorem}
The LP algorithm solves the Equitable Content Spread Maximization problem with an expected optimization value:
\begin{equation}
E[ECS_{APPROX}] \geq (1-1/e)ECS_{OPT}
\end{equation}
And LP solves the Equitable Content Spread Maximization problem with an expected equity between groups:
\begin{equation}
(1-1/e)/2 \leq E[EQUITY_{APPROX}] \leq 2/(1-1/e)
\end{equation}
\end{theorem}

\begin{proof}
The optimization value from the linear program is greater than or equal to the optimal value for the integer problem, as values considered for $y_j$ in equation \ref{lp-constraint} are a superset of the values in IP definition. The proof uses additional values: a real number selection for the an edge $e_j$ determined by the linear program $y_j^*$, and the corresponding indicators for a node $v_i$ at distance $r$, $x_{ir}^*$. The result of randomized rounding on the values $y_j^*$ produces the rounded integer values for each edge $e_j$, $y_j^+$. From the rounded edge value, the associated value of whether a node $i$ is reachable by a path of at most $r$ given the rounded edge values is $x_{ir}^+$.
\begin{multline}
    E[x_{ir}^+] = 1 - \prod_{j \in P_{ir}}(1 - y_j^*)
    \geq 1 - \prod_{j \in P_{ir}}e^{-y_k^*} = 1 - e^{\sum_{j \in P_{ir}} -y_k^*}\\ 
    \geq 1 - e^{-x_{ij}^*}\geq (1 - 1/e)x_{ij}^*
\end{multline}
For any $x_{ir}^*$ value found by the linear program, after rounding, the expected value of $x_ir^+$ is $\geq (1-1/e)$ times the optimal value for $x_{ir}$.

\begin{flalign}
    &E[ECS_{APPROX}] = \sum_r\sum_i \mu_r*w_i*E[x_{ir}^+] \\
    &\geq (1-1/e)\sum_r\sum_i \mu_r*w_i*x_{ir}^* \\
    &\geq (1-1/e)ECS_{OPT}
\end{flalign}
    
% \end{multline*}


Or the overall approximation is expected to be $\geq (1-1/e)ECS_{OPT}$ .

It is also possible to produce an upper bound on the expected value.

\ian{there's an issue with this proof. It apparently should be 2e, but I don't see how?}
\begin{multline}
    E[x_{ir}^+] = 1 - \prod_{j \in P_{ir}}(1 - y_j^*)\leq 1 - \prod_{j \in P_{ir}}e^{-2y_k^*} = 1 - e^{\sum_{j \in P_{ir}} -2y_k^*} \\
     \geq 1 - e^{-2x_{ij}^*} \geq 1 - (1 - 2x_{ij}^*)= 2x_{ij}^*
\end{multline}
    
% \end{flalign*}

The expected $x_{ir}^+$ found by the program is no more than 2 times the optimal value for $x_{ir}$.

The equity equation from the Linear Program can also be presented as a ratio, similar to the initial equity definition. In this format, the LP relaxation version of the equity is:

\begin{equation}
{ \sum_r\sum_{l \in g_1}{\mu_r*w_l*x_{lr}}/|g_1| \over \sum_r\sum_{l \in g_2}{\mu_r*w_l*x_{lr}}/|g_2|} = 1
\end{equation}

With a lower bound and upper bound for for $x_{lr}$, we can rewrite the inequality as follows.

\begin{align*}
 &{\sum_r{\sum_{l \in g_1}\mu_r*w_l*(1-1/e)x_{lr}/|g_1|}} \over {\sum_r{\sum_{l \in g_2}\mu_r*w_l*2x_{lr}/|g_2|}}\\
 \leq &{\sum_r{\sum_{l \in g_1}\mu_r*w_l*E[x_{lr}^+]/|g_1|}} \over {\sum_r{\sum_{l \in g_2}{\mu_r*w_l*E[x_{lr}^+]}/|g_2|}} \\
 \leq &{\sum_r{\sum_{l \in g_1}\mu_r*w_l*2x_{lr}/|g_1|}} \over {\sum_r{\sum_{l \in g_2}\mu_r*w_l*(1-1/e)x_{lr}/|g_2|}}
\end{align*}

or the expected equity is bound by $(1-1/e)/2 \leq E[EQUITY_{APPROX}] \leq 2/(1-1/e)$.

\end{proof}

\section{Practical Optimizations}

\stitle{Constraint Reduction}
The LP-Advanced algorithm has is inefficient because it has as many constraints as the number of nodes times the diameter of the network. To reduce the number of constraints, we take the approach of removing variables which would have no impact on the output. Particularly we look for two types of variables where based on the equation are defined as equal to one or equal to zero.

A variable which represents a path to a node for which there is an equal or shorter path in the initial graph is inherently defined as equal to one. For every edge, a path of this length is guaranteed, or in other words in the corresponding linear program the $x_{ir}$ variable is $\leq$ the summation of every edge's indicator variable. There should be no optimal edge selection where this variable is not set to one. These variables are then irrelevant to the maximization function, as they are a constant offset. However, a single "placeholder" variable is used for each group for the equity calculations. These variables are bounded equal to one, and are multiplied by the content to each group relative to the group size for each equity calculation.

Additionally, a variable which represents a path to a node for which the node can never be reached in that distance is inherently defined as equal to zero. If for every edge possibly added to the graph, the node can still not be reached in a path of that length, then in the corresponding linear program the $x_{ir}$ is $\leq$ 0, meaning it can take no value other than zero. In this case, the variables are inconsequential to every equation within the calculation, and can be removed from the equation with no consequence.

\begin{algorithm}[t]
\small
    \caption{ Linear Program Optimized (LP-OPT)}\label{algo:LP}
    \hspace*{\algorithmicindent} \textbf{Input} : $G(V, E), V_s, E_c, KPerNode, \mathcal{G}, Directed, SortValue$\\
    \hspace*{\algorithmicindent} \textbf{Output} : Approximate Equitable Content Spread Edge Selection
    \begin{algorithmic}[1]
        \State{$SD \leftarrow$ 
        MULTIPLE-SOURCES-SHORTEST-DISTANCES $(G, V_s)$}
        \State{$E_c \leftarrow e_{u,v} \in E $ | $ SD(u) + 1 < SD(v)$}
        \State{$\forall_{e_j \in E_c}  SD\Delta_j \leftarrow $ EDGE-DELTA-SINGLE$(G, SD, e_j)$}
        \State{$NodeValues \leftarrow \{\}$}
        \State{$EdgeConstraints \leftarrow \{\}$}
        \For{$v_i \in V$}
            \State $r_{min} \leftarrow MIN(SD\Delta[Node])$
            \For{$r \leftarrow r_{min}; r < SD[Node]; r \leftarrow r + 1$}
                \State $NodeValues.Append(x_{i,r})$
                \State $EdgeConstriants[i,r] \leftarrow \{\}$
            \EndFor
        \EndFor
        
        \For{$P_{i,r} \in EdgeConstraints$}
            \For{$SD\Delta_j \in DP\Delta$}
                \If{$SD\Delta_k[i] \leq r$}
                    \State{$EdgeConstraints[i,r].Append(j)$}
                \EndIf
            \EndFor
        \EndFor
        
        \State{$NodeNeighbors \leftarrow \{\}$}
        \State{$\forall_{v_i \in V} NodeNeighbors[i] \leftarrow \{\}$}
        \For{$e_{u,v} \in E_c$}
            \State{$NodeNeighbors[u].Append(e_{u,v})$}
            \If{$!Directed$}
                \State{$NodeNeighbors[v].Append(e_{u,v})$}
            \EndIf
        \EndFor 
        \State{$y^* \leftarrow $ Solve the LP For Edge Weights, using Node Values, Edge Constraints, KPerNode, Node Neighbors, and $\mathcal{G}$}
        \State4\{$Roundings \leftarrow []$
        \For {$iter \leftarrow 0; iter < 200; iter \leftarrow iter + 1$}
            \State{$E_p \leftarrow \{\}$}
            \For {$j \leftarrow 0; j < |E_c|; j \leftarrow j + 1$}
                \If{RANDOM$(0,1) < y_j^*$}
                    \State{$E_p.Insert(e_j)$}
                \EndIf
            \EndFor
            \State{$RoundingSD\Delta \leftarrow $EDGE-DELTA-MULTIPLE$(G, SD, E_p)$}
            \State{$Disparity \leftarrow 0$}
            \For{$G_1, G2_2 \in \mathcal{G}$}
                \State{$CSG_1 \leftarrow \sum_{v_j \in G_1} F_(E_p, v_j)*w_j/|G_1|$ given $RoundingSD\Delta$}
                \State{$CSG_2 \leftarrow \sum_{v_j \in G_2} F_(E_p, v_j)*w_j/|G_2|$ given $RoundingSD\Delta$}
                \State $d \leftarrow Max(CSG_1/CSG_2, CSG_2/CSG_1) - 1$
                \State{$Disparity = Max(Disparity, d)$}
            \EndFor
            \State{$CS \leftarrow \sum_{v_j \in V} F_(E_p, v_j)*w_j$ given $RoundingSD\Delta$}
            \State{$Roundings.Append({Disparity, CS, E_p})$}
        \EndFor
        \State{Sort Roundings, by Disparity, Ascending}
        \State{$TopK \leftarrow Roundings[0:SortValue]$}
        \State{Sort TopK, by Content Spread, Descending}
        \State{$E_p \leftarrow TopK[0]$}\\
        \Return{$E_p$}
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\small
    \caption{ Difference Graphs (DIFF)}\label{algo:sp-delta}
    \hspace*{\algorithmicindent} \textbf{Input} : G(V, E), SD, Queues\\
    \hspace*{\algorithmicindent} \textbf{Output} : Node Distances 
    Deltas
    \begin{algorithmic}[1]
        \State diff $= \{\}$
        \State $i \leftarrow 0$
        \While{$i < Max(Queues.Keys())$}
            \If{$i \not\in Queues.Keys()$}
                \State $i \leftarrow i + 1$
                \State Continue
            \EndIf
            \State $Queue \leftarrow Queues[i]$
            \While{$Length(Queue) > 0$}
                \State $Node \leftarrow Queue.Pop()$
                \If{$Node \in $ diff $|| SD[Node] < i$}
                    \State Continue
                \EndIf
                \State diff$[Node] \leftarrow i$
                \For{$Neighbor \in G.Neighbors(Node)$}
                    \If {$i+1 \not\in Queues$}
                        \State $Queues[i+1] \leftarrow \{\}$
                    \EndIf
                    \State $Queues[i+1].PushBack(Neighbor)$
                \EndFor
            \EndWhile
            \State $i \leftarrow i + 1$
        \EndWhile
        \Return diff
    \end{algorithmic}
\end{algorithm}
\begin{algorithm}[t]
\small
    \caption{Edge Delta, Single (EDGE-DELTA-SINGLE)}\label{algo:edge-delta-sing}
    \hspace*{\algorithmicindent} \textbf{Input} : $G(V, E), SD, e_{u,v}$\\
    \hspace*{\algorithmicindent} \textbf{Output} : Node Distances Delta for e
    \begin{algorithmic}[1]
    \State $Queues \leftarrow \{\}$
    \State $Queues[SD(u)+1] = \{v\}$\\
    \Return{DIFF$(G, SD, Queues)$}
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\small
    \caption{Edge Delta, Multiple (EDGE-DELTA-MULTIPLE)}\label{algo:edge-delta-mult}
    \hspace*{\algorithmicindent} \textbf{Input} : $G(V, E), SD, E_\Delta$\\
    \hspace*{\algorithmicindent} \textbf{Output} : Node Distances Delta for e
    \begin{algorithmic}[1]
    \State $Queues \leftarrow \{\}$
    \For{$e_{u,v} \in E_\Delta$}
        \If{$SD(u)+1 \not\in Queues$}
            \State $Queues[SD(u)+1] = \{v\}$
        \Else
            \State $Queues[SD(u)+1].Append(v)$
        \EndIf
    \EndFor
    \Return{DIFF$(G, SD, Queues)$}
    \end{algorithmic}
\end{algorithm}


\stitle{Difference Graphs}
With a considerably faster LP Solver, the recalculation of shortest distances can become the dominating factor in the algorithm. However, the shortest distances needed to be computed are many repeated shortest distances calculations on an initial graph, with the modification of a set of one or many new edges being added. Accordingly, we were able to calculate "differences" in shortest distances based on the addition of new edges.

To find the difference in shortest distances, we perform a graph search based on the existing distances and the updated distances. Throughout the graph search, we maintain a set of queues, with each queue being the distance to the current node. We initialize these queues with the values from the new edges: the destination of the new edge is added to the queues with the value of the distance of the source of the edge, incremented by one. At this point all of the potential new starting nodes are added to the multi-queue. We then start at the lowest queue (distance 1) and process each node on the queue until the queue is empty, and then proceed to the next queue. When processing the node, we keep a running tally of the "difference" which is a map of nodes to their new distances. With each node coming off the queue, if there is a smaller distance in either the existing graphs distances, or in the difference map, then the node is ignored and processing goes onto the next node. Otherwise the node is added to the difference map with the value from the queue, and it's neighbors are added to the queue with the current queue's value plus one, and then the node is removed and the next node in the queue is processed. When every queue has been processed, the resulting difference map is returned. In practice, this solution will have significantly less nodes to process than a BFS which much process every node and every edge, since this process will only consider subgrapghs around destination nodes which have a distance less than the updated distance.

In our algorithm this method is used in two ways. First, in rounding it is used over the set of new edges being added to compute the graph differences which can then be used to update the MIP score, both for Content Spread and Equity, without recomputing the MIP. To do this, it simply needs to take the existing MIP score, and for each node in the difference, subtract the probability associated with the shortest distance, and add the probability as if it had the distance in the difference. Additionally, in preprocessing the difference on each edge generates the $x_{ir}$ values on which the edge has a distance shorter than the existing shortest distance. These values are easily inverted, yielding the $P_{ir}$ sets. With these optimizations, we found that the preprocessing and rounding were equal or less in the resources necessary to finish computation when compared with the LP solver.

\begin{algorithm}[t]
\small
    \caption{Iterative Linear Program (LP-ITER)}\label{algo:lp-iter}
    \hspace*{\algorithmicindent} \textbf{Input} : $G(V, E), V_s, E_c, k, \mathcal{G}, Directed, SortValue, \alpha$\\
    \hspace*{\algorithmicindent} \textbf{Output} : Approximate Equitable Content Spread Edge Selection
    \begin{algorithmic}[1]
    \State{$E_p^* \leftarrow \{\}$}
    \State{$SD \leftarrow$ 
    MULTIPLE-SOURCES-SHORTEST-DISTANCES $(G, V_s)$}
    \State{$E_c \leftarrow e_{u,v} \in E $ | $ SD(u) + 1 < SD(v)$}

    \State{$NodeNeighbors \leftarrow \{\}$}
    \State{$\forall_{v_i \in V} NodeNeighbors[i] \leftarrow \{\}$}
    \For{$e_{u,v} \in E_c$}
        \State{$NodeNeighbors[u].Append(e_{u,v})$}
        \If{$!Directed$}
            \State{$NodeNeighbors[v].Append(e_{u,v})$}
        \EndIf
    \EndFor
    
    \State{$KPerNode \leftarrow \{\}$}
    \For{$v_i \in V$}
        \State{$KPerNode[i] \leftarrow k$}
    \EndFor
    \State{$Target \leftarrow |\{v_u \in V$ | $\exists e_{u,x} \in E_c\}|$}
    \State{$FeasibleNodes \leftarrow Target$}
    \While{$FeasibleNodes > \alpha*Target$}
        \State{$E_p \leftarrow $LP-OPT$(G(V,E+E_p^*), V_s, E_c, KPerNode, \mathcal{G},$}
        
        $Directed, SortValue)$
        \If{$|E_p| == 0$}
            \Return{$E_p^*$}
        \EndIf
        \State{$E_p^*.AddAll(E_p)$}
        \For{$e_u,w \in E_p$}
            \State{$KPerNode[u] \leftarrow KPerNode[u]-1$}
            \If{$!Directed$}
                \State{$KPerNode[v] \leftarrow KPerNode[v]-1$}
            \EndIf
        \EndFor
        \State{$FeasibleNodes \leftarrow |\{v_i \in V | KPerNode[i] > 0, $ }
        
        $NodeNeighbors[i] > 0\}|$
    \EndWhile
    \Return{$E_p^*$}    
    \end{algorithmic}
    
\end{algorithm}

==> future.tex <==
\new{\section{Future Work}\label{sec:future-work}}

\new{One extension for the work above is for multiple types of content, where each individual both creates and desires each type of content to some degree. This relationship can be shown as a tripartite graph such as in Figure~\ref{fig:tri-content}, with each individual appearing both as a generator and consumer on the graph, connected to each content type by a weight indicating the amount of content produced on a topic, or the desire to consume content on that topic. Content spread is then measured for each individual as the sum of content received over all topics, multiplied by the weight of interest in each topic for that individual. The fairness constraint is then modified to guarantee that across each demographic group, the content spread as defined by the weighted sum for individuals of content over topics should be equal between demographic groups. To solve the Fair Multi Topic Content Spread Maximization Problem, the fairness constraint must be met, and then the overall content spread (as defined by weighted content to each individual on each topic) should be maximized. We leave this problem open for future works.}

\new{Another extension considers the possibility that not every edge suggestion will be accepted. It is assumed there is some probability that an individual will accept an edge suggestion $p_e$. Given an edge recommendation set $E_p$, each subset $\bold{e}$ appears with the probability $\prod_{e \in \bold{e}}p_e \prod_{e \in E_p - \bold{e}}(1-p_e)$. Accordingly, the expected content spread to each node is the content spread from each set $\bold{e}$ times the probability that $\bold{e}$ is the actual accepted set. The fairness constraint for this problem is that the expected content to each group is equal, based on the probability of each set $\bold{e}$. Considering there is an exponential number of sets $\bold{e} \in 2^{|E_p|}$, it is infeasible to calculate every possible set, and approximating over this power set becomes fundamental to calculating the probabilistic content spread and satisfying the fairness constraint. This problem is also to be addressed in future works.}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=.35\textwidth]{figs/bipartite content.PNG}
%     \vspace{-4mm}
%     \caption{\new{The tripartite graph showing the relationship between individuals producing content and individuals desiring content across a variety of topics.}}
%     \label{fig:tri-content}
%     \vspace{-4mm}
% \end{figure}

==> plots.tex <==
%2D
\begin{figure*}[!tb] % 1
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\textwidth]{plots/bfVsLpapprox-disparity.pdf}
        \vspace{-8mm}\caption{demonstration of near optimal disparity of $\LP$-Approx}
        \label{fig:optimal-disparity}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\textwidth]{plots/bfVsLpapprox-lift.pdf}
        \vspace{-8mm}\caption{demonstration of near optimal lift of $\LP$-Approx}
        \label{fig:optimal-lift}
    \end{minipage}
    \hfill
    % \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/lpVsContinous_disparity.pdf}
    %     \vspace{-8mm}\caption{$\LP$-Advanced v.s. Cont. Greedy in disparity on small graphs at various k}
    %     \label{fig:bl-varyk-disp}
    % \end{minipage}
    % \hfill
    %     \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/lpVsContinous_lift.pdf}
    %     \vspace{-8mm}\caption{$\LP$-Advanced v.s. cont. Greedy in lift on small graphs at various k}
    %     \label{fig:bl-varyk-lift}
    % \end{minipage}

\end{figure*}

% \begin{figure*}[!tb] % 2
    % \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/lpVsContinous_time.pdf}
    %     \vspace{-8mm}\caption{$\LP$-Advanced v.s. cont. Greedy in time on small graphs at various k}
    %     \label{fig:bl-varyk-time}
    % \end{minipage}\hfill
    %     \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/varying_sources_FOF.pdf}
    %     \vspace{-8mm}\caption{\new{$\LP$-Advanced v.s. cont. Greedy in disparity on small graphs at various \# of content nodes in Friend of Friend model}}
    %     \label{fig:bl-varysource-disparity}
    % \end{minipage} \hfill
    % \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/varying_sources_comm.pdf}
    %     \vspace{-8mm}\caption{\new{$\LP$-Advanced v.s. cont. Greedy in disparity on small graphs at various \# of content nodes in Intersecting Group Count model}}
    %     \label{fig:bl-varysource-disparity-community}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/lpVsContinous_sources_lift.pdf}
    %     \vspace{-8mm}\caption{$\LP$-Advanced v.s. cont. Greedy in lift on small graphs at various \# of content nodes}
    %     \label{fig:bl-varysource-lift}
    % \end{minipage}
%     \vspace{-3mm}
% \end{figure*}

% \begin{figure*}[!tb] % 3
%     \begin{minipage}[t]{0.23\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{plots/lpVsContinous_sources_time.pdf}
%         \vspace{-8mm}\caption{$\LP$-Advanced v.s. cont. Greedy on time on small graphs at various \# of content nodes}
%         \label{fig:bl-varysoure-time}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.23\linewidth}
%         \centering
%                 \includegraphics[width=\textwidth]{plots/comparison-threeAlgo-disparity.pdf}
%         \vspace{-8mm}\caption{\scalable v.s. $\LP$-Advanced v.s. cont. Greedy on disparity}
%         \label{fig:compare-disparity}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.23\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{plots/comparison-threeAlgo-lift.pdf}
%         \vspace{-8mm}\caption{\scalable v.s. $\LP$-Advanced v.s. cont. Greedy on the lift}
%         \label{fig:compare-lift}
%     \end{minipage}
%         \hfill
%     \begin{minipage}[t]{0.23\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{plots/comparison-threeAlgo-time.pdf}
%         \vspace{-8mm}\caption{\scalable v.s. $\LP$-Advanced v.s. cont. Greedy on time} \label{fig:compare-time}
%     \end{minipage}
%     \vspace{-3mm}
% \end{figure*}


\begin{figure*}[!tb]
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\textwidth]{plots/forest-fire-disparity.pdf}
        \vspace{-8mm}\caption{Disparity of \scalable for diff. \# nodes per iteration}
        \label{fig:ff-disparity}
    \end{minipage}
    \hfill
    \vspace{-3mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\textwidth]{plots/forest-fire-lift.pdf}
        \vspace{-8mm}\caption{the lift of the \scalable for diff. \# nodes per iteration}
        \label{fig:ff-lift}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\textwidth]{plots/forest-fire-time.pdf}
        \vspace{-8mm}\caption{the runtime of the \scalable for diff. \# nodes per iteration}
        \label{fig:ff-time}
    \end{minipage}
    \hfill
    % \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/scaling-disparity.pdf}
    %     \vspace{-8mm}\caption{the disparity achieved by the \scalable algorithm at various scales}
    %     \label{fig:scale-disparity}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.23\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{plots/scaling-Time.pdf}
    %     \vspace{-8mm}\caption{the runtime of the \scalable algorithm at various scales\abol{change the y-axis to log-scale}}
    %     \label{fig:scale-runtime}
    % \end{minipage}
    \vspace{-3mm}
\end{figure*}

% \begin{figure*}
%     \begin{minipage}[t]{0.23\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{plots/scaling-lift.pdf}
%         \vspace{-8mm}\caption{the lift achieved by the \scalable algorithm at various scales}
%         \label{fig:scale-lift}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.23\linewidth}
%     \centering
%     \includegraphics[width=\textwidth]{plots/scaling-Time.pdf}
%         \vspace{-8mm}\caption{the runtime of the \scalable algorithm as the number of nodes increase to half a million}
%         \label{fig:scale-runtime}
%     \end{minipage}
%     \vspace{-3mm}
% \end{figure*}



% \begin{figure*}[!tb]
    
% \end{figure*}
